User Positioning in mmW 5G Networks using Beam-RSRP Measurements and Kalman Filtering

In this paper, we exploit the 3D-beamforming features of multiantenna equipment employed in fifth generation (5G) networks, operating in the millimeter wave (mmW) band, for accurate positioning and tracking of users. We consider sequential estimation of users' positions, and propose a two-stage extended Kalman filter (EKF) that is based on reference signal received power (RSRP) measurements. In particular, beamformed downlink (DL) reference signals (RS) are transmitted by multiple base stations (BSs) and measured by user equipmentn(UE) employing receive beamforming. The so-obtained BRSRP measurements are fed back to the BS where the corresponding direction-of-departure are sequentially estimated by a novel EKF. Such angle estimates from multiple BSs are subsequently fused on a central entity into 3D position estimates of UE by means of an angle-based EKF. The proposed positioning scheme is scalable since the computational burden is shared among different network entities, namely transmission/reception points (TRPs) and 5G-NR Node B (gNB), and may be accomplished with the signalling currently specified for 5G. We assess the performance of the proposed algorithm on a realistic outdoor 5G deployment with a detailed ray tracing propagation model based on the METIS Madrid map. Numerical results with a system operating at 39 GHz show that sub-meter 3D positioning accuracy is achievable in future mmW 5G networks.

==> CRLB.tex <==
\section{Cram\'er-Rao Bound}

The \gls{CRB} is a lower bound on the estimation variance of any unbiased estimator and it is defined as the inverse of the \gls{FIM} of the likelihood function describing the observations. In this section we first show that the distribution of \gls{BRSRP} measurements approaches a Gaussian for a growing number of subcarriers. The \gls{FIM} on the \gls{DoD} of the \gls{DL} \gls{LoS} path is then found based on Gaussian distributed \gls{BRSRP} measurements. Finally, the \gls{FIM} on the \gls{UE} location is provided.

\subsection{Distribution of BRSRP Measurements} \label{sec:brsrp_dist}

Recall that $\beta_{i,j}$ denotes \gls{BRSRP} measurements. It can be shown that $\mathcal{M}_{f} \beta_{i,j}$ follows a noncentral $\chi^2$-distribution with $2\mathcal{M}_f$ degrees-of-freedom and noncentrality parameter $\lambda_{i,j} = \sum_m^{\mathcal{M}_f} |[\bm{s}]_m [\bm{b}_f]_m \gamma_{i,j}|^2$ \cite{PZJD17},\cite[Ch.2]{PS08}. Here, $\gamma_{i,j} = \bm{b}_{\mathrm{UE}}^{i^T}(\vartheta_a,\varphi_a) \bm{\Gamma} \bm{b}_{\mathrm{BS}}^j(\vartheta_d,\varphi_d)$. The \gls{pdf} of $\beta_{i,j}$ is then \cite{PZJD17},\cite[Ch.2]{PS08}
\begin{align} \label{eq:chi_squared}
p(\beta_{i,j}) & = \frac{\mathcal{M}_f}{\tilde{\sigma}_{i,j}^2}\left(\frac{\mathcal{M}_f\beta_{i,j}}{\lambda_{i,j}}\right)^{\frac{\mathcal{M}_f-1}{2}} \mathrm{e}^{-\frac{\lambda_{i,j}+\mathcal{M}_f\beta_{i,j}}{\tilde{\sigma}_{i,j}^2}} \nonumber\\ & \qquad I_{\mathcal{M}_f-1}\left(\frac{2\sqrt{\lambda_{i,j}\mathcal{M}_f\beta_{i,j}}}{\tilde{\sigma}_{i,j}^2}\right)
\end{align}
where $I_x(\cdot) \in \mathbb{R}$ denotes a modified Bessel function of the first kind. For growing $\mathcal{M}_f$ the \gls{pdf} in \eqref{eq:chi_squared} approaches a Gaussian \cite{PZJD17,HM13}, and we thus have $\beta_{i,j} \sim \mathcal{N}(\mu_{i,j},\sigma_{i,j}^2)$, where the mean and variance are given by $\mu_{i,j} = \lambda_{i,j}/\mathcal{M}_f + \tilde{\sigma}_{i,j}^2$ and $\sigma_{i,j}^2 =  \tilde{\sigma}_{i,j}^4/\mathcal{M}_f + 2\tilde{\sigma}_{i,j}^2 \lambda_{i,j}/\mathcal{M}_f^2$, respectively. It then follows that both mean and variance of \gls{BRSRP} measurements have information regarding the \gls{DoD}.

Let us define the \gls{SNR} of the $(i,j)$ beam pair as $\mathrm{SNR}_{i,j} \triangleq \lambda_{i,j}/\tilde{\sigma}^2_{i,j}$. It is instructive to note that the information carried by the variance of \gls{BRSRP} measurements on the \gls{DoD} starts becoming insignificant when $\mathrm{SNR}_{i,j} < \mathcal{M}_f/2$. However, if $\mathrm{SNR}_{i,j} \ll \mathcal{M}_f/2$ the accuracy of the \gls{DoD} estimates degrade significantly. Neglecting the information carried by the variance of \gls{BRSRP} measurements regarding the \gls{DoD} simplifies significantly the estimation procedure but the cost is increased estimation variance and biased estimates.

Let $\bm{\beta}\in\mathbb{R}^{\mathcal{M}_\mathrm{BS}}$ denote the \gls{RSRP} measurements for all \gls{BS} beams and a given \gls{UE} beam. The chosen \gls{UE} beam is the one that yields the largest sum of \gls{BS}' \gls{RSRP} measurements among all \gls{UE} beams, i.e. $\max_i \sum_{j=1}^{\mathcal{M}_\mathrm{BS}} \beta_{i,j}$. It follows that $\bm{\beta} \sim \mathcal{N}(\bm{\mu}(\bm{\Theta}),\bm{C}(\bm{\Theta}))$, where
\begin{align} \label{eq:gaussian_approx_brsrp}
\bm{\mu}(\bm{\Theta}) & = \bm{A}(\vartheta,\varphi) \bm{\alpha}\frac{P_{\mathrm{Tx}}}{\mathcal{M}_f} + \bm{1} \tilde{\sigma}^2 \\ \bm{C}(\bm{\Theta}) & = \mathrm{diag}\left\{\bm{A}(\vartheta,\varphi) \bm{\alpha} \frac{2\tilde{\sigma}^2}{\mathcal{M}_f} + \bm{1} \frac{\tilde{\sigma}^4}{\mathcal{M}_f} \right\},
\end{align}
where $\bm{\Theta}=[\vartheta,\varphi,\alpha_1,\alpha_4,\Re\{\alpha_2\},\Im\{\alpha_2\},\tilde{\sigma}^2]^T$ denotes the unknown parameter vector. Moreover, $\bm{\alpha} = \mathrm{vec}\{\bm{\Gamma}^H \bm{b}^{i^\ast}_{\mathrm{UE}}(\vartheta,\varphi) \bm{b}^{i^T}_{\mathrm{UE}}(\vartheta,\varphi)\bm{\Gamma}\}$, $P_{\mathrm{Tx}} = \sum_m^{\mathcal{M}_f} |[\bm{s}]_m [\bm{b}_f]_m|^2$, and $\bm{A}(\vartheta,\varphi)\in\mathbb{C}^{\mathcal{M}_{\mathrm{BS}} \times 4}$ is given by
\begin{align}
\bm{A}(\vartheta,\varphi) & = [\bm{b}^\ast_{\mathrm{BS}_\phi}(\vartheta,\varphi) \odot \bm{b}_{\mathrm{BS}_\phi}(\vartheta,\varphi)\; \bm{b}^\ast_{\mathrm{BS}_\theta}(\vartheta,\varphi) \odot \bm{b}_{\mathrm{BS}_\phi}(\vartheta,\varphi)\nonumber \\ & \bm{b}^\ast_{\mathrm{BS}_\phi}(\vartheta,\varphi) \odot \bm{b}_{\mathrm{BS}_\theta}(\vartheta,\varphi)\; \bm{b}^\ast_{\mathrm{BS}_\theta}(\vartheta,\varphi) \odot \bm{b}_{\mathrm{BS}_\theta}(\vartheta,\varphi)].
\end{align}
Here $\odot$ denotes the Hadamard-Schur (element-wise) product. 
%In case the Electric-field corresponding to both \gls{BS} beams and \gls{UE} beams is single-polarized (e.g., $b^i_{\mathrm{UE}_\phi} = b^j_{\mathrm{BS}_\phi}= 0$), $\bm{\alpha}$ is then a scalar ($\bm{\alpha}=\alpha$) and $\bm{A}(\vartheta,\varphi) = \bm{b}^\ast_{\mathrm{BS}_\theta}(\vartheta,\varphi) \odot \bm{b}_{\mathrm{BS}_\theta}(\vartheta,\varphi)$. A similar result is obtained when the Electric-field corresponding to either \gls{BS} beams or \gls{UE} beams is single-polarized and the channel does not introduce any depolarization (i.e., $\bm{\Gamma}$ is diagonal), such as for the \gls{LoS} path.
Fig.~\ref{fig:hist_pdf} illustrates the histogram of \gls{RSRP} measurements as well as the Gaussian approximation in \eqref{eq:gaussian_approx}. Results show that the distribution of \gls{RSRP} measurements approaches a Gaussian for increasing number of subcarriers. Similarly, such a Gaussian distribution can be assumed even for a single subcarrier for increasing received \gls{SINR}.

\begin{figure}[!t]
    \centering
    \begin{subfigure}{0.47\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/hist_pdf_mf1_10mW.eps}
        \caption{}
        \label{}
    \end{subfigure}
    \begin{subfigure}{0.47\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/hist_pdf_mf1_100mW.eps}
        \caption{}
        \label{}
    \end{subfigure}  
%    \\[12pt]
    \begin{subfigure}{0.47\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/hist_pdf_mf100_10mW.eps}
        \caption{}
        \label{}
    \end{subfigure}
        \begin{subfigure}{0.47\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{figs/hist_pdf_mf1000_10mW.eps}
        \caption{}
        \label{}
    \end{subfigure}  
    \caption{Histogram of \gls{RSRP} measurements and corresponding Gaussian \gls{pdf} approximation. (a) single subcarrier and \SI{10}{\deci\bel\milli} \gls{Tx} power budget. (b) single subcarrier and \SI{20}{\deci\bel\milli} \gls{Tx} power budget. (c) $100$ subcarriers and \SI{10}{\deci\bel\milli} \gls{Tx} power budget. (d) $1000$ subcarriers and \SI{10}{\deci\bel\milli} \gls{Tx} power budget. The distribution of \gls{RSRP} measurements approach a Gaussian for increasing number of subcarriers. A Gaussian distribution for the \gls{RSRP} measurements can be assumed even for a single subcarrier for increasing received \gls{SINR}.}
    \label{fig:hist_pdf}
\end{figure}

\subsection{Fisher Information Matrix of the \gls{DoD}}

Let us now assume that $\bm{\beta} \sim \mathcal{N}(\bm{\mu}(\bm{\Theta}),\bm{C}(\bm{\Theta}))$. The \gls{FIM} for Gaussian distributed observations is given by \cite[Ch.3]{Kay93}
\begin{align} \label{eq:fim_dod}
    & [\bm{\mathcal{I}}(\bm{\Theta})]_{m,n} = \frac{\partial \bm{\mu}^T(\bm{\Theta})}{\partial \bm{\Theta}_m} \bm{C}^{-1}(\bm{\Theta}) \frac{\partial \bm{\mu}(\bm{\Theta})}{\partial \bm{\Theta}_n^T} \nonumber \\
    & \qquad + \frac{1}{2} \mathrm{tr}\left\{\bm{C}^{-1}(\bm{\Theta}) \frac{\partial \bm{C}(\bm{\Theta})}{\partial \bm{\Theta}_m} \bm{C}^{-1}(\bm{\Theta}) \frac{\partial \bm{C}(\bm{\Theta})}{\partial \bm{\Theta}_n}\right\}.
\end{align}
The lower-bound on the estimation variance of the \gls{DoD} is then obtained from the $(2\times2)$ upper-left block of $\bm{\mathcal{I}}^{-1}(\bm{\Theta})$.

\subsection{Fisher Information Matrix of the \gls{UE} Location}

The \gls{FIM} of the \gls{UE}'s location can be found by first considering a distribution for the estimated \glspl{DoD}. In particular, we assume that
\begin{equation} \label{eq:dod_dist}
    \begin{bmatrix}
    \hat{\vartheta}_k\\ \hat{\varphi}_k
    \end{bmatrix} \sim \mathcal{N}\left(\begin{bmatrix}
    \vartheta_k\\ \varphi_k
    \end{bmatrix},\bm{C}_k(\vartheta_k,\varphi_k)\right),
\end{equation}
where the subscript $k$ denotes the \gls{BS} index. The assumption in \eqref{eq:dod_dist} is a good approximation of the estimates obtained by the \gls{MLE}; see next Section. It is well-known that the \gls{MLE} is asymptotically Gaussian distributed, asymptotically unbiased, and its asymptotic covariance matrix attains that of the \gls{CRB}, under general regularity conditions on the likelihood function \cite[Ch.10]{CB02}. We thus assume that $\bm{C}_k(\vartheta_k,\varphi_k)\in\mathbb{R}^{2\times2}$ equals the $(2\times2)$ upper-left block of $\bm{\mathcal{I}}^{-1}(\bm{\Theta})$.

Let $\bm{m}\in\mathbb{R}^{2K}$ denote the estimated \glspl{DoD} of $K$ \glspl{BS} to a \gls{UE}. It follows that $\bm{m}\sim\mathcal{N}\left(\bm{\mu}(\bm{p}),\bm{C}(\bm{p})\right)$, where
\begin{align}
    \bm{\mu}(\bm{p}) & = \left[\vartheta_1(\bm{p}),\varphi_1(\bm{p}),\ldots,\vartheta_K(\bm{p}),\varphi_K(\bm{p})\right]^T \\
    \bm{C}(\bm{p}) & = \mathrm{blkdiag}\left\{\bm{C}_1(\bm{p}),\ldots,\bm{C}_K(\bm{p})\right\}.
\end{align}
Here, $\bm{p}\in \mathbb{R}^{3}$ denotes the $3$D Cartesian coordinate of a \gls{UE}'s position and $\mathrm{blkdiag}\{\cdot\}$ denotes a block-diagonal matrix. Note that 
\begin{align}
    \vartheta_k(\bm{p}) & =\arctan\left(\frac{-\Delta z_k}{d_{{2D}_k}}\right)+\pi/2\\
    \varphi_k(\bm{p}) & =\arctan2\left(\Delta y_k,\Delta x_k\right),
\end{align}
where $d_{{2D}_k} = \sqrt{\Delta x^2_k+\Delta y^2_k}$, $\Delta x_k=x_\mathrm{UE}-x_{\mathrm{BS}_k}$, $\Delta y_k=y_\mathrm{UE}-y_{\mathrm{BS}_k}$, and $\Delta z_k=z_\mathrm{UE}-z_{\mathrm{BS}_k}$. The \gls{FIM} of $\bm{p}$ is then given by \cite[Ch.3]{Kay93}
\begin{align} \label{eq:fim_pos}
    [\bm{\mathcal{I}}(\bm{p})]_{m,n} & = \frac{\partial \bm{\mu}^T(\bm{p})}{\partial \bm{p}_m} \bm{C}^{-1}(\bm{p}) \frac{\partial \bm{\mu}(\bm{p})}{\partial \bm{p}_n^T} \nonumber \\
    & + \frac{1}{2} \mathrm{tr}\left\{\bm{C}^{-1}(\bm{p}) \frac{\partial \bm{C}(\bm{p})}{\partial \bm{p}_m} \bm{C}^{-1}(\bm{p}) \frac{\partial \bm{C}(\bm{p})}{\partial \bm{p}_n}\right\}.
\end{align}
The \gls{CRB} on the \gls{UE}'s position $\bm{p}$ from estimated \glspl{DoD} is $\bm{\mathcal{I}}(\bm{p})^{-1}$.

%and $\bm{C}\in\mathbb{R}^{2K\times2K}$ the corresponding covariance matrix. They are given by $\bm{m} = [\hat{\vartheta}_1,\hat{\varphi}_1,\ldots,\hat{\vartheta}_K,\hat{\varphi}_K]^T$ and $\bm{C}=\mathrm{blkdiag}\{\bm{C}_1,\ldots,\bm{C}_K\}$, respectively. Here, $\mathrm{blkdiag}\{\cdot\}$ denotes a block-diagonal matrix.
%Let also $\bm{p}\in\mathbb{R}^{3}$ denote the $3$D position of the \gls{UE}. The log-likelihood function of $\bm{p}$ is then
%\begin{align} \label{eq:llf_pos}
%    \ell(\bm{p}|\bm{m}) & = -\frac{K}{2} \ln 2\pi-\frac{1}{2}\ln\det\{\bm{C}\}\nonumber \\
%    & \quad - \frac{1}{2}(\bm{m}-\bm{\mu}(\bm{p}))^T \bm{C}^{-1} (\bm{m}-\bm{\mu}(\bm{p})),
%\end{align}
%where $\bm{\mu}(\bm{p})\in\mathbb{R}^{2K}$ is given by
%\begin{align}
%    \bm{\mu}(\bm{p}) & = \Bigg[\arctan\left(\frac{d_{{2D}_1}}{\Delta z_1}\right),\arctan\left(\frac{\Delta y_1}{\Delta x_1}\right),\nonumber\\
%    & \ldots,\arctan\left(\frac{d_{{2D}_K}}{\Delta z_K}\right),\arctan\left(\frac{\Delta y_K}{\Delta x_K}\right)\Bigg]^T.
%\end{align}
%Here, $d_{{2D}_k} = \sqrt{\Delta x^2_K+y^2_K}$, $\Delta x_k=x_\mathrm{UE}-x_{\mathrm{BS}_k}$, $\Delta %y_k=y_\mathrm{UE}-y_{\mathrm{BS}_k}$, and $\Delta z_k=z_\mathrm{UE}-z_{\mathrm{BS}_k}$. 

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> commented_bibitems.tex <==
% % Article within a journal
% @ARTICLE{koon,
% 	author  = {Koonin, E V and Altschul, S F and P Bork}, 
% 	title   = {BRCA1 protein products: functional motifs}, 
% 	journal = {Nat Genet}, 
% 	year    = {1996},
% 	volume  = {13}, 
% 	pages   = {266-267}
% }	

% % Article within a journal supplement
% @ARTICLE{oreg,
% 	author  = {Orengo, C A and Bray, J E and Hubbard, 
% 		   T and LoConte, L and Sillitoe, I}, 
% 	title   = {Analysis and assessment of ab initio 
% 		   three-dimensional prediction, secondary 
% 		   structure, and contacts prediction},
% 	journal = {Proteins}, 
% 	year    = {1999},
% 	volume  = {Suppl 3}, 
% 	pages   = {149-170}
% }	

% % In press article
% @inpress{khar,
% 	author  = {Kharitonov, S A and Barnes, P J}, 
% 	title   = {Clinical aspects of exhaled nitric oxide},
% 	journal = {Eur Respir J}, 
% 	note    = {in press} 
% }	

% %
% % Published abstract
% %
% @ARTICLE{zvai,
% 	author  = {Zvaifler, N J and Burger, J A and Marinova-Mutafchieva, 
% 		   L and Taylor, P and Maini, R N},
% 	title   = {Mesenchymal cells, stromal derived factor-1 and 
% 		   rheumatoid arthritis [abstract]},
% 	journal = {Arthritis Rheum}, 
% 	year    = {1999},
% 	volume  = {42}, 
% 	pages   = {s250},
% }	


% %
% % Article within conference proceedings
% %
% @Inproceedings{xjon,
% 	author    = {X Jones}, 
% 	title     = {Zeolites and synthetic mechanisms},
% 	booktitle = {Proceedings of the First National Conference on 
% 		     Porous Sieves: 27-30 June 1996; Baltimore},
% 	year      = {1996},
% 	  editor  = {Y Smith}, 
% 	  pages   = {16-27},
% 	  organization  = {Stoneham: Butterworth-Heinemann}
% }	

% %%%%%%%%
% %  Book chapter, or article within a book
% %
% @incollection{schn,
% 	author    = {E Schnepf}, 
% 	title     = {From prey via endosymbiont to plastids: 
% 		     comparative studies in dinoflagellates},
% 	booktitle = {Origins of Plastids}, 
% 	editor    = {R A Lewin}, 
% 	publisher = {Chapman and Hall},
% 	pages     = {53-76}, 
% 	year      = {1993},
% 	  address = {New York}, 
% 	  volume  = {2}, 
% 	  edition = {2nd} 
% }	

% %%%%%%%%
% % Whole issue of journal
% %
% @wholejournal{pond,
% 	editor  = {B Ponder and S Johnston and L Chodosh}, 
% 	title   = {Innovative oncology},
% 	journal = {Breast Cancer Res}, 
% 	year  = {1998},
% 	  volume= {10}, 
% 	  pages = {1-72}
% }	


% %%%%%%%%
% % Whole conference proceedings
% %
% @proceedings{smith,
% 	editor  = {Y Smith}, 
% 	title   = {Proceedings of the First National Conference
% 		   on Porous Sieves: 27-30 June 1996; Baltimore},
% 	year = 1996,
% 	  address= {Stoneham}, 
% 	  publisher = {Butterworth-Heinemann},
% }	


% %%%%%%%%
% % Complete book
% %
% @book{marg,
% 	author    = {L Margulis}, 
% 	title     = {Origin of Eukaryotic Cells},
% 	publisher = {Yale University Press}, 
% 	year      = {1970},
% 	address   = {New Haven} 
% }



% %%%%%%%%
% % Monograph or book in series 
% %
% @incollection{hunn,
% 	author    = {G W Hunninghake and J E Gadek}, 
% 	title     = {The alveloar macrophage},
% 	booktitle = {Cultured Human Cells and Tissues},
% 	publisher = {Academic Press}, 
% 	year      = {1995},
%   pages      = {54-56},
% 	  editor   = {T J R Harris}, 
% 	  address  = {New York}, 
% 	  note     = {Stoner G (Series Editor): Methods and Perspectives in Cell Biology, vol 1} 
% }


% %%%%%%%%
% % Book with institutional author
% @manual{advi,
% 	  title   = {Annual Report}, 
% 	    organization  = {Advisory Committee on Genetic Modification}, 
% 	    address = {London},
% 	    year    = {1999}
% }


% %%%%%%%%
% % PHD Thesis
% %
% @phdthesis{koha,
% 	author = {R Kohavi}, 
% 	title  = {Wrappers for performance enhancement and
% 		  obvious decision graphs},
% 	school = {Stanford University, Computer Science Department},
% 	year   = {1995}
% }

% %%%%%%%%
% % Webpage Link / URL
% %
% @webpage{mouse,
% 	title  = {The Mouse Tumor Biology Database},
% 	url = {http://tumor.informatics.jax.org/cancer\_links.html}
% }


==> mle.tex <==
\section{Maximum Likelihood Estimation} \label{sec:mle}

\subsection{MLE of DoDs}

Under the Gaussian assumption for the \gls{BRSRP} measurements the log-likelihood function of $\bm{\Theta}$ is
\begin{align} \label{eq:log-likelihood}
    \ell(\bm{\Theta}|\bm{\beta}) & = -\frac{\mathcal{M}_{\mathrm{BS}}}{2} \ln{2\pi} -\frac{1}{2} \ln{\mathrm{det}\{\bm{C}(\bm{\Theta})\}} \nonumber\\
    & - \frac{1}{2}(\bm{\beta}-\bm{\mu}(\bm{\Theta}))^T \bm{C}^{-1}(\bm{\Theta})(\bm{\beta}-\bm{\mu}(\bm{\Theta})).
\end{align}
The \gls{MLE} is then given by
\begin{equation} \label{eq:mle}
    \hat{\bm{\Theta}}_{\mathrm{MLE}} = \arg \max_{\bm{\Theta}} \ell(\bm{\Theta}|\bm{\beta}).
\end{equation}

Gradient based optimization techniques are typically employed for solving \eqref{eq:mle}. Convenient expressions for the gradient of \eqref{eq:log-likelihood} can be found in \cite[Ch.3]{Kay93}. Next, we propose an approximate \gls{MLE} that can be used for initializing such a numerical optimization technique.


%We consider a Levenberg-Marquardt approach for solving \eqref{eq:mle}. In particular, such an algorithm guarantees convergence to a local optima, and in case the initialization is close to the global optima, the maximum of the likelihood function is found. The gradient of \eqref{eq:log-likelihood} is \cite{Kay93}
%\begin{align}
%    \frac{\partial \ell(\bm{\Theta}|\bm{\beta})}{\partial [\bm{\Theta}]_n} & = -\frac{1}{2} \mathrm{tr}\left\{\bm{C}^{-1}(\bm{\Theta}) \frac{\partial \bm{C}(\bm{\Theta})}{\partial [\bm{\Theta}]_n}\right\} + \frac{\partial \bm{\mu}^T(\bm{\Theta})}{\partial [\bm{\Theta}]_n} \bm{C}^{-1}(\bm{\Theta}) (\bm{\beta}-\bm{\mu}(\bm{\Theta}))\nonumber\\
%    & \quad - \frac{1}{2}(\bm{\beta}-\bm{\mu}(\bm{\Theta}))^T\frac{\partial \bm{C}^{-1}(\bm{\Theta})}{\partial [\bm{\Theta}]_n}(\bm{\beta}-\bm{\mu}(\bm{\Theta})),
%\end{align}
%where \cite{Kay93}
%\begin{equation}
%    \frac{\partial \bm{C}^{-1}(\bm{\Theta})}{\partial [\bm{\Theta}]_n} = -\bm{C}^{-1}(\bm{\Theta}) \frac{\partial \bm{C}(\bm{\Theta})}{\partial [\bm{\Theta}]_n}\bm{C}^{-1}(\bm{\Theta})
%\end{equation}

\subsection{Approximate MLE of DoDs}

We now consider a low \gls{SNR} approximation of the \gls{MLE} that is useful in finding initial estimates for gradient based optimization of the log-likelihood function in \eqref{eq:log-likelihood}. Recall from Section \ref{sec:brsrp_dist} that when $\mathrm{SNR}<\mathcal{M}_f/2$ the variance of \gls{BRSRP} measurements starts becoming dominated by the measurement noise variance $(\tilde{\sigma}^2)$ and insensitive to changes in angles. Hence, in the low \gls{SNR} regime it suffices to consider the mean of \gls{BRSRP} measurements in order to estimate the \gls{DoD}. In other words, we assume that $\bm{\beta} \sim \mathcal{N}(\bm{\mu}(\bm{\Theta}),\sigma^2\bm{I}))$ where $\sigma^2$ is an unknown nuisance parameter. The corresponding approximate log-likelihood function of $(\bm{\Theta},\sigma^2)$ is then
\begin{align} \label{eq:log-likelihood_approx}
    \ell_\mathrm{aprx}(\bm{\Theta},\sigma^2|\bm{\beta}) & = -\frac{\mathcal{M}_\mathrm{BS}}{2} \ln{2\pi} -\frac{\mathcal{M}_\mathrm{BS}}{2} \ln{\sigma^2} \nonumber \\ 
    & \hspace{2cm} - \frac{1}{2\sigma^2}\|\bm{\beta}-\bm{\mu}(\bm{\Theta}))\|^2.
\end{align}

Since $\mathbb{E}\left\{\frac{\partial^2\ell_\mathrm{aprx}(\bm{\Theta},\sigma^2|\bm{\beta})}{\partial \bm{\Theta} \partial \sigma^2}\right\} = 0$ one may decouple the estimation of $\bm{\Theta}$ from that of $\sigma^2$. Hence, we can focus on
\begin{equation} \label{eq:sep_nlls}
    \hat{\bm{\Theta}} = \arg \min_{\bm{\Theta}} \|\bm{\beta}-\bm{\mu}(\bm{\Theta})\|^2.
\end{equation}
Moreover, since $\bm{\mu}(\bm{\Theta})$ can be written as (see \eqref{eq:gaussian_approx_brsrp})
\begin{align}
    \bm{\mu}(\bm{\Theta}) & = \left[\bm{A}(\vartheta,\varphi) \frac{P_{\mathrm{Tx}}}{\mathcal{M}_f}, \, \bm{1}\right] \; [\bm{\alpha}^T, \, \tilde{\sigma}^2]^T,
\end{align}
and by noting that \eqref{eq:sep_nlls} is a separable \gls{NLLS} problem \cite{GP03}, it follows that 
\begin{align} \label{eq:mle_angle_aprx}
    (\hat{\vartheta},\hat{\varphi}) & = \arg \min_{(\vartheta,\varphi)} \|\bm{P}^\bot_{A 1}(\vartheta,\varphi) \bm{\beta}\|^2 \\
    \begin{bmatrix} \hat{\alpha}\\\hat{\tilde{\sigma}}^2
    \end{bmatrix} & = \left[\bm{A}(\vartheta,\varphi) \frac{P_{\mathrm{Tx}}}{\mathcal{M}_f}, \, \bm{1}\right]^\dag \bm{\beta}.
\end{align}
Here, $(\cdot)^\dag$ denotes the Moore-Penrose pseudo-inverse. Moreover, $\bm{P}^\bot_{A 1}(\vartheta,\varphi)=\bm{I}-\bm{P}_{A 1}(\vartheta,\varphi)$, and $\bm{P}_{A 1}(\vartheta,\varphi)\in\mathbb{R}^{\mathcal{M}_\mathrm{BS}\times\mathcal{M}_\mathrm{BS}}$ denotes an orthogonal projection matrix. We note that $\bm{P}_{A 1}(\vartheta,\varphi) = \bm{\mathcal{P}}_{A}(\vartheta,\varphi) + \bm{\mathcal{P}}_{1}$, where $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ and $\bm{\mathcal{P}}_{1}$ denote oblique projection matrices. In particular, the range-space of $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ is spanned by the columns of $\bm{A}(\vartheta,\varphi)$ while its nullspace contains a subspace spanned by vector $\bm{1}$. Similarly, the range-space of $\bm{\mathcal{P}}_{1}$ is spanned by vector $\bm{1}$ while its nullspace contains a subspace spanned by the columns of $\bm{A}(\vartheta,\varphi)$ \cite{BS94}.

%The derivative of $\ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})$ \gls{wrt} $\sigma^2$ and $\bm{\alpha}$ are given, respectively, by
%\begin{align}
%    \frac{\partial \ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})}{\partial \sigma^2} & =  \bm{1}^T(\bm{\beta}-\bm{A}(\vartheta,\varphi)\bm{\alpha} - \bm{1}\sigma^2) \\
%    \frac{\partial \ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})}{\partial \bm{\alpha}} & = (\bm{A}^H(\vartheta,\varphi)(\bm{\beta}-\bm{1}\sigma^2-\bm{A}(\vartheta,\varphi),\bm{\alpha}))^\ast,
%\end{align}
%where we have neglected constant terms, and $c^\ast$ denotes the complex-conjugate of $c$. Equating the above derivatives to zero, and solving for $\sigma^2$ and $\bm{\alpha}$ with substitution, yields \begin{align}
%    \hat{\bm{\alpha}} & = \bm{A}^\dag(\hat{\vartheta},\hat{\varphi}) \bm{\mathcal{P}}_{A}(\hat{\vartheta},\hat{\varphi}) \bm{\beta} \label{eq:alpha_hat} \\
%    \hat{\tilde{\sigma}}^2 & = \frac{\bm{1}^T \bm{\mathcal{P}}^\bot_{A}(\hat{\vartheta},\hat{\varphi}) \bm{\beta}}{\mathcal{M}_\mathrm{BS}}. \label{eq:sigma2_hat}
%\end{align}
%Moreover, using \eqref{eq:alpha_hat} and \eqref{eq:sigma2_hat} in \eqref{eq:log-likelihood_approx}, and neglecting constant terms, results in
%\begin{equation} \label{eq:mle_angle_aprx}
%    (\hat{\vartheta},\hat{\varphi}) = \arg \min_{(\vartheta,\varphi)} \|\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) \bm{\beta}\|^2 - \frac{(\bm{1}^T\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) \bm{\beta})^2}{\mathcal{M}_\mathrm{BS}}.
%\end{equation}
%Here, $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi)\in\mathbb{R}^{\mathcal{M}_\mathrm{BS} \times \mathcal{M}_\mathrm{BS}}$ denotes an oblique projection matrix that is given by $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) = \bm{I}-\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$. In particular, $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ is also an oblique projection matrix and it is given by
%\begin{equation} \label{eq:oblique_proj}
%\bm{\mathcal{P}}_{A}(\vartheta,\varphi) = \bm{A}(\vartheta,\varphi)(\bm{A}^H(\vartheta,\varphi)\bm{P}^\bot_{\bm{1}}\bm{A}(\vartheta,\varphi))^{-1} \bm{A}^H(\vartheta,\varphi) \bm{P}^\bot_{\bm{1}},
%\end{equation}
%where $\bm{P}^\bot_{\bm{1}} = \bm{I}-\frac{1}{\mathcal{M}_\mathrm{BS}}\bm{1}\bm{1}^T$ denotes an orthogonal projection matrix with nullspace spanned by vector $\bm{1}$. We note that both $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi)$ and $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ are idempotent by not symmetric matrices. We also note that the column-space of $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ is spanned by the columns of $\bm{A}(\vartheta,\varphi)$ and the corresponding nullspace contains a subspace spanned by vector $\bm{1}$ \cite{BS94}. The results in \eqref{eq:alpha_hat}-\eqref{eq:mle_angle_aprx} may be understood as filtering-out a bias term from the measurements that is confined to a (known) subspace disjoint of that of the transmitted signal.

\subsection{MLE of UE Position}

Given that the estimated \glspl{DoD} are Gaussian distributed the log-likelihood function of $\bm{p}$ is
\begin{align} \label{eq:llf_pos}
    \ell(\bm{p}|\bm{m}) & = -K \ln 2\pi-\frac{1}{2}\ln\det\{\bm{C}(\bm{p})\}\nonumber \\
    & \quad - \frac{1}{2}(\bm{m}-\bm{\mu}(\bm{p}))^T \bm{C}^{-1}(\bm{p}) (\bm{m}-\bm{\mu}(\bm{p})).
\end{align}
The \gls{MLE} of the \gls{UE} position is then
\begin{equation} \label{eq:mle_pos}
    \hat{\bm{p}}_{\mathrm{MLE}} = \arg \max_{\bm{p}} \ell(\bm{p}|\bm{m}).
\end{equation}

Next, a simple closed-form algorithm is proposed for finding an initial estimate of the \gls{UE} position. This facilitates in finding the global optimum of \eqref{eq:llf_pos}.

\subsection{Initial Estimate of UE Position}

Let $\{\hat{\vartheta}_k,\hat{\varphi}_k\}_{k=1}^{K}$ denote the estimated \glspl{DoD} at $K$ \glspl{BS}. A simple way of determining the \gls{UE} $3$D position from angles consists in finding the ranges between \glspl{BS} and \gls{UE} by means of triangulation. Mathematically, such a problem can be formulated as follows
\begin{equation}
\left(\bm{D} + \bm{\epsilon}_1\right) \bm{r} = \tilde{\bm{p}}_\mathrm{BS} + \bm{\epsilon}_2,
\label{eq:tls_pos}
\end{equation}
where $\bm{r}\in\mathbb{R}^{K^2-K}$ denotes the (unknown) ranges, and $\bm{D} \in \mathbb{R}^{3(K^2-K)/2 \times (K^2-K)}$ and $\tilde{\bm{p}}_\mathrm{BS} \in \mathbb{R}^{3(K^2-K)/2}$ are given by
\begin{subequations}
\begin{align}
\bm{D} & = \begin{bmatrix}
\bm{D}_{1,2} & \bm{0} & \cdots \\
\bm{0} & \bm{D}_{1,3} & \cdots \\
\vdots & \vdots & \ddots
\end{bmatrix} \\
\tilde{\bm{p}}_\mathrm{BS} & = [\tilde{\bm{p}}_{1,2}^T, \tilde{\bm{p}}_{1,3}^T \ldots]^T.
\end{align}
\end{subequations}
Here, $\tilde{\bm{p}}_{n,m}\in\mathbb{R}^{3}$ denotes the difference between the positions of the $n$th and $m$th anchors while $\bm{D}_{n,m}\in\mathbb{R}^{3 \times 2}$ is given by
\begin{equation}
\bm{D}_{n,m} = \begin{bmatrix}
\sin(\hat{\vartheta}_n) \cos(\hat{\varphi}_n) & -\sin(\hat{\vartheta}_m) \cos(\hat{\varphi}_m)\\
\sin(\hat{\vartheta}_n) \sin(\hat{\varphi}_n) & -\sin(\hat{\vartheta}_m) \sin(\hat{\varphi}_m)\\
\cos(\hat{\vartheta}_n) & -\cos(\hat{\vartheta}_m)
\end{bmatrix}.
\end{equation}
It is important to note that the error vectors $\bm{\epsilon}_1 \in \mathbb{R}^{3(K^2-K)/2}$and $\bm{\epsilon}_2 \in \mathbb{R}^{3(K^2-K)/2}$ in \eqref{eq:tls_pos} model the estimation errors in $\{\hat{\vartheta}_k,\hat{\varphi}_k\}_{k=1}^{K}$ and the uncertainty (common in practice) in the \glspl{BS} positions, respectively. Solving \eqref{eq:tls_pos} for $\bm{r}$ can be accomplished under a \gls{TLS} framework\footnote{A least-squares solution would be appropriate if $\bm{\epsilon}_1 = \bm{0}$.}, where the minimum-norm solution is found as follows \cite[Ch. 6]{GL13}
\begin{enumerate}
\item Let $\bm{\mathcal{D}} \triangleq \left[\bm{D}, \, \tilde{\bm{p}}_\mathrm{BS}\right]$, and find the right singular-vectors of $\bm{\mathcal{D}}$, denoted by $\bm{\mathcal{V}}\in\mathbb{R}^{(K^2-K+1) \times (K^2-K+1)}$.
\item Let $\bm{v} \in \mathbb{R}^{K^2-K + 1}$ denote the right singular-vector corresponding to the smallest singular value.
\item The \gls{TLS} estimate of the range vector is
\begin{equation}
\hat{\bm{r}} = [\bm{v}]_{K^2-K+1}^{-1} \tilde{\bm{v}},
\end{equation}
where $\tilde{\bm{v}}\in\mathbb{R}^{K^2-K}$ contains all but the last element of $\bm{v}$.
\item The initial estimate of the \gls{UE}'s $3$D position is then
\begin{subequations}
\begin{align}
\hat{\bm{p}}_k & = [\hat{\bm{r}}]_{k}[\sin(\hat{\vartheta}_k) \cos(\hat{\varphi}_k) \, \sin(\hat{\vartheta}_k) \sin(\hat{\varphi}_k) \nonumber \\ & \qquad \cos(\hat{\vartheta}_k)]^T+\bm{p}_{\mathrm{BS}_k}, \\
\hat{\bm{p}} & = \mathrm{median}\left(\hat{\bm{p}}_1,\,\ldots,\,\hat{\bm{p}}_{K^2-K}\right).
\end{align}
\end{subequations}
\end{enumerate}

==> mle_init.tex <==
\section{Approximate MLE}

We now consider a low \gls{SNR} approximation of the \gls{MLE} that is useful in finding initial estimates for gradient based optimization of the log-likelihood function in \eqref{eq:log-likelihood}. Recall from Section \ref{sec:brsrp_dist} that when $\mathrm{SNR}<\mathcal{M}_f/2$ the variance of \gls{BRSRP} measurements starts becoming dominated by the measurement noise variance $(\tilde{\sigma}^2)$ and insensitive to changes in angles. Hence, in the low \gls{SNR} regime it suffices to consider the mean of \gls{BRSRP} measurements in order to estimate the \gls{DoD}. In other words, we assume that $\bm{\beta} \sim \mathcal{N}(\bm{\mu}(\bm{\Theta}),\sigma^2\bm{I}))$ where $\sigma^2$ is an unknown nuisance parameter. The corresponding approximate log-likelihood function of $\bm{\Theta}$ is then
\begin{equation} \label{eq:log-likelihood_approx}
    \ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta}) = -\frac{\mathcal{M}_\mathrm{BS}}{2} \ln{2\pi} -\frac{\mathcal{M}_\mathrm{BS}}{2} \ln{\sigma^2} - \frac{1}{2\sigma^2}\|\bm{\beta}-\bm{\mu}(\bm{\Theta}))\|^2.
\end{equation}

The derivative of $\ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})$ \gls{wrt} $\tilde{\sigma}^2$ and $\bm{\alpha}$ are given, respectively, by \cite{Kay93}
\begin{align}
    \frac{\partial \ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})}{\partial \tilde{\sigma}^2} & =  \bm{1}^T(\bm{\beta}-\bm{A}(\vartheta,\varphi)\bm{\alpha} - \bm{1}\tilde{\sigma}^2) \\
    \frac{\partial \ell_\mathrm{aprx}(\bm{\Theta}|\bm{\beta})}{\partial \bm{\alpha}} & = (\bm{A}^H(\vartheta,\varphi)(\bm{\beta}-\bm{1}\tilde{\sigma}^2-\bm{A}(\vartheta,\varphi),\bm{\alpha}))^\ast,
\end{align}
where we have neglected constant terms and $c^\ast$ denotes the complex-conjugate of $c$. Equating the above derivatives to zero, and solving for $\tilde{\sigma}^2$ and $\bm{\alpha}$ with substitution, yields \begin{align}
    \hat{\bm{\alpha}} & = \bm{A}^\dag(\hat{\vartheta},\hat{\varphi}) \bm{\mathcal{P}}_{A}(\hat{\vartheta},\hat{\varphi}) \bm{\beta} \label{eq:alpha_hat} \\
    \hat{\tilde{\sigma}}^2 & = \frac{\bm{1}^T \bm{\mathcal{P}}^\bot_{A}(\hat{\vartheta},\hat{\varphi}) \bm{\beta}}{\mathcal{M}_\mathrm{BS}}. \label{eq:sigma2_hat}
\end{align}
Moreover, using \eqref{eq:alpha_hat} and \eqref{eq:sigma2_hat} in \eqref{eq:log-likelihood_approx}, and neglecting constant terms, results in
\begin{equation} \label{eq:mle_angle_aprx}
    (\hat{\vartheta},\hat{\varphi}) = \arg \min_{(\vartheta,\varphi)} \|\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) \bm{\beta}\|^2 - \frac{(\bm{1}^T\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) \bm{\beta})^2}{\mathcal{M}_\mathrm{BS}}.
\end{equation}
Here, $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi)\in\mathbb{R}^{\mathcal{M}_\mathrm{BS} \times \mathcal{M}_\mathrm{BS}}$ denotes an oblique projection matrix that is given by $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi) = \bm{I}-\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$. In particular, $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ is also an oblique projection matrix and it is given by
\begin{equation} \label{eq:oblique_proj}
\bm{\mathcal{P}}_{A}(\vartheta,\varphi) = \bm{A}(\vartheta,\varphi)(\bm{A}^H(\vartheta,\varphi)\bm{P}^\bot_{\bm{1}}\bm{A}(\vartheta,\varphi))^{-1} \bm{A}^H(\vartheta,\varphi) \bm{P}^\bot_{\bm{1}},
\end{equation}
where $\bm{P}^\bot_{\bm{1}} = \bm{I}-\frac{1}{\mathcal{M}_\mathrm{BS}}\bm{1}\bm{1}^T$ denotes an orthogonal projection matrix with nullspace spanned by vector $\bm{1}$. We note that both $\bm{\mathcal{P}}^\bot_{A}(\vartheta,\varphi)$ and $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ are idempotent by not symmetric matrices. We also note that the column-space of $\bm{\mathcal{P}}_{A}(\vartheta,\varphi)$ is spanned by the columns of $\bm{A}(\vartheta,\varphi)$ and the corresponding nullspace contains a subspace spanned by vector $\bm{1}$ \cite{BS94}. The results in \eqref{eq:alpha_hat}-\eqref{eq:mle_angle_aprx} may be understood as filtering-out a bias term from the measurements that is confined to a subspace disjoint from that of the signal of interest of the spans a known subspace is but otherwise unknown
